Video Person Re-identification by Temporal Residual Learning

In this paper, we propose a novel feature learning framework for video person re-identification (re-ID). The proposed framework largely aims to exploit the adequate temporal information of video sequences and tackle the poor spatial alignment of moving pedestrians. More specifically, for exploiting the temporal information, we design a temporal residual learning (TRL) module to simultaneously extract the generic and specific features of consecutive frames. The TRL module is equipped with two bi-directional LSTM (BiLSTM), which are respectively responsible to describe a moving person in different aspects, providing complementary information for better feature representations. To deal with the poor spatial alignment in video re-ID datasets, we propose a spatial-temporal transformer network (ST^2N) module. Transformation parameters in the ST^2N module are learned by leveraging the high-level semantic information of the current frame as well as the temporal context knowledge from other frames. The proposed ST^2N module with less learnable parameters allows effective person alignments under significant appearance changes. Extensive experimental results on the large-scale MARS, PRID2011, ILIDS-VID and SDU-VID datasets demonstrate that the proposed method achieves consistently superior performance and outperforms most of the very recent state-of-the-art methods.

==> checklab.tex <==
 % Making those `Label(s) have changed\dots' messages more explicit
%
% The \LaTeX{} kernel produces the messages when something, while the
% |.aux| file is being scanned (after the \cs{AtEndDocument} tokens
% have been executed), sets the \cs{if@tempswa} switch with the
% command \cs{@tempswatrue}.
%
% (This fact can be used by packages, such as my |footmisc.sty|, to
% piggy-back on the message; but it's nice in that circumstance and
% others to be sure where the message is coming from.)
%
% This is a jiffy patch to the kernel so that it produces a
% (\cs{typeout}) message for each label \emph{it} thinks has changed.
%
% Usage: Incorporate this code into a package or class file,       or
%        \input this file from a package or class file,            or
%        \makeatletter \input{checklab} \makeatother in your document
%                                                    preamble
%
% This software jiffy is placed in the public domain.  Do with it as
% you wish, though I have to say I would prefer you not to claim it
% as your own (otoh, it's the product of a twisted mind, so probably
% not an attractive thing to claim).
%
% Robin Fairbairns (rf10@cl.cam.ac.uk)
% Produced in this form 1999/01/15
%
\def\@testdef #1#2#3{%
  \def\reserved@a{#3}%
  \expandafter \ifx \csname #1@#2\endcsname \reserved@a
  \else
    \@tempswatrue
    \typeout{label change: #1@#2 was
      \expandafter \ifx \csname #1@#2\endcsname \relax
        unset
      \else
        \csname#1@#2\endcsname\space
      \fi
      now #3}%
  \fi
}

